LDM: Large Tensorial SDF Model for Textured Mesh Generation

Previous efforts have managed to generate production-ready 3D assets from text or images. However, these methods primarily employ NeRF or 3D Gaussian representations, which are not adept at producing smooth, high-quality geometries required by modern rendering pipelines. In this paper, we propose LDM, a novel feed-forward framework capable of generating high-fidelity, illumination-decoupled textured mesh from a single image or text prompts. We firstly utilize a multi-view diffusion model to generate sparse multi-view inputs from single images or text prompts, and then a transformer-based model is trained to predict a tensorial SDF field from these sparse multi-view image inputs. Finally, we employ a gradient-based mesh optimization layer to refine this model, enabling it to produce an SDF field from which high-quality textured meshes can be extracted. Extensive experiments demonstrate that our method can generate diverse, high-quality 3D mesh assets with corresponding decomposed RGB textures within seconds.

==> sections/algorithm01.tex <==
\begin{algorithm}
\caption{Your algorithm's name}
\begin{algorithmic}[1] % The number tells LaTeX to number each line
\Procedure{YourProcedureName}{parameters}
\State \textbf{Initialize:} Your initialization
\While{condition}
    \State operation 1
    \State operation 2
    \If{condition}
        \State operation 3
    \EndIf
\EndWhile
\State \Return result
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> tables/ablations_views_flx.tex <==

\begin{table}
\setlength{\tabcolsep}{1.4mm}
\caption{Ablation on txxxxxx}
\begin{tabular}{c|c|c|c|c|c|c}
    \Xhline{0.8pt}
    Probes  &Reference &MLP & 6890  & 689  & 69  & 5  \\
    \Xhline{0.8pt}
    PSNR↑     &-  &12.91   & \textbf{25.73} &25.46   & 24.69        & 23.38  \\
    SSIM↑    &-  &0.697    &\textbf{0.959}  &0.947   & 0.937       & 0.922  \\
    Time/$ms$ &$83.980$  &4.329 & $0.368$  & $0.236$   & $0.220$     & $\textbf{0.216}$  \\
    \Xhline{0.8pt}
\end{tabular}
\label{tab:visbility}  
\end{table}

==> tables/feature_comp.tex <==



\begin{table}
\centering
\setlength{\tabcolsep}{0.8mm}
\caption{ The features of different methods, our framework provides comprehensive feature support. Our method is the only one that provides illumination decoupling (Illum. dec.). }
\begin{tabular}{l|cccc}
\hline
Method      & \multicolumn{1}{l}{Text to 3d} & \multicolumn{1}{l}{Image to 3d} & \multicolumn{1}{l}{Representation} & \multicolumn{1}{l}{Illum. dec.} \\ \hline
LRM         & $\times$               & \checkmark              & NeRF                & $\times$                                    \\
LGM         & \checkmark                 &\checkmark             & 3DGS                  & $\times$                                     \\
CRM         & $\times$                     & \checkmark                   & SDF                        &  $\times$      \\   
Instand3d   & \checkmark               & \checkmark                & NeRF                 &  $\times$                                  \\

Ours        & \checkmark               & \checkmark                 & TensoSDF                   & \checkmark                       \\ \hline
\end{tabular}
\label{tab: featurecomp}
\end{table}

% InstantMesh & $\times$                   & \checkmark                  & NeRF+SDF                    &  $\times$                          \\

==> tables/image_compare.tex <==

\begin{table}[]
\centering
\setlength{\tabcolsep}{0.75mm}
\caption{Quantitative results demonstrate that the color and geometric quality of the 3D assets generated by our method outperforms other methods. }
\begin{tabular}{l|ccccc}
\Xhline{0.8pt}
             & PSNR ↑  & SSIM ↑   & LPIPS ↓    & Chamfer Dist. ↓  & Vol. IoU ↑        \\ \hline
One-2-3-45 & 18.93     & 0.779    & 0.166       & 0.0614  & 0.4126               \\
CRM & 21.59       & 0.864   & 0.159            & 0.0335  & 0.4213               \\
OpenLRM   & 20.29   & 0.829    & 0.186              & 0.0482   & 0.3731                  \\
LGM        & 20.05   & 0.798     & 0.176        & 0.0417   & 0.4331                 \\
Ours         & \textbf{22.52} & \textbf{0.873} & \textbf{0.143}  & \textbf{0.0241}  & \textbf{0.4361}     \\ 

\Xhline{0.8pt}
\end{tabular}
\label{tab:delit compare}
\end{table}



==> tables/text-compare.tex <==

\begin{table}[]
\setlength{\tabcolsep}{6.75mm}
\caption{\todo{xxxx} }
\begin{tabular}{l|cc}
\Xhline{0.8pt}
             & CLIP-Sim ↑  & User-Pref. ↑         \\ \hline
Shap-E  & 18.33     & 0.206                   \\
One-2-3-45  & 19.23     & 0.211                   \\
Ours         & \textbf{21.32} & \textbf{0.583}    \\


\Xhline{0.8pt}
\end{tabular}
\label{tab:delit compare}
\end{table}


